Kardar-Parisi-Zhang Universality, Anomalous Scaling and Crossover Effects in the Growth of Cdte Thin Films

We report on the growth dynamic of CdTe thin films for deposition temperatures ($T$) in the range of $150\,^{\circ}\mathrm{C}$ to $300\,^{\circ}\mathrm{C}$. A relation between mound evolution and large-wavelength fluctuations at CdTe surface has been established. One finds that short-length scales are dictated by an interplay between the effects of the formation of defects at boundaries of neighbouring grains and a relaxation process which stems from the diffusion and deposition of particles (CdTe molecules) torward these regions. A Kinetic Monte Carlo model corroborates these reasonings. As $T$ is increased, the competition gives rise to different scenarios in the roughening scaling such as: uncorrelated growth, a crossover from random to correlated growth and transient anomalous scaling. In particular, for $T = 250\,^{\circ}\mathrm{C}$, one shows that surface fluctuations are described by the celebrated Kardar-Parisi-Zhang (KPZ) equation, in the meantime that, the universality of height, local roughness and maximal height distributions for the KPZ class is, finally, experimentally demonstrated. The dynamic of fluctuations at the CdTe surface for other temperatures still is described by the KPZ equation, but with different values for the superficial tension ($\nu$) and excess of velocity ($\lambda$). Namely, for $T = 150\,^{\circ}\mathrm{C}$ one finds a Poissonian growth that indicates $\nu = \lambda = 0$. For $T = 200\,^{\circ}\mathrm{C}$, however, a Random-to-KPZ crossover is found, with $\lambda > 0$ in the second regime. Finally, for films grown at $T = 300\,^{\circ}\mathrm{C}$, one demonstrates that a KPZ growth with $\lambda < 0$ takes place. We discuss the different mechanisms leading to KPZ scaling which depend on $T$, and conjecture the behavior of the phenomenological parameter $\lambda$ as function of the deposition temperature.

==> titulo/Acknowledgments.tex <==
The conclusion of this dissertation coincides with the end of a
long special period in my life, which goes beyond of physics. Thus,
I think it is appropriate to start thanking those people who have helped me at 
both directions since the beginning of this journey. My parents are my basis. An integral 
part of what I am today is why I have been learning, through examples, that true, passion and 
faith must guide our attitudes, even when all the world seems to behave conversely. Thanks for 
all support and motivation, mainly in difficult times. I also must thanks Miriam Santos for 
so many years of accomplicity. It will be impossible to forget them...

I am enormously grateful to my supervisors, Sukarno Ferreira and Tiago Oliveira. Sukarno is a great experimentalist. He knows almost everything about any growth and characterization technique, as well knows a lot 
about electronic. However, the most remarkable in Sukarno is his personality, 
always open to teach, advise, and help young and expert physicists. Fortunately, I was ``adopted'' by him since the beginning of my undergraduate and today I am proud of 
finishing this MSc under his supervision.
% Additionally, he always supported me to participate of workshops, 
% including that one about KPZ held in Kyoto, Japan, where I could meet inspirational people and make new friends. 
In the same vein, Tiago is ``just'' the most competent person that I have known. His
criticism has played a crucial role in my progress as a physicist and it is very clear that without it, 
this work could be just more one containing several meaningless exponents. Additionally, Tiago has been showing me, as matter
of example, a great ``scientific integrity'', a lack in many unprepared people that share the 
authorship in papers by convenience, instead merit. I am grateful to both for supporting my level change towards the Doctorate,
as well as my adventure in Japan.

By the way, I would like to thank Prof. S. Ferreira for sharing that adventure with me. ``Thank'' for leaving me lost in the middle of Kyoto one day before my talk, without a map ... at the end
of the day (or at the beginning), I was able to give a good talk. 
Many thanks also for recommending me to an abroad PhD. The KPZ workshop was a great experience. I am glad to meet J. Krug, T. Halpin-Healy, J. Kim, K. Takeuchi, M. Myllys, P. Yunker, P. Ferrari... 
and so many inspirational physicists and mathematicians. The former two have given important insights about my work, as well as wise advices about my academic plans. It was a privilege to receive them. About P. Yunker, I hope that we can work together soon. \textit{Muchas gracias} to my friends J. Rodriguez-Laguna, Silvia N. Santalla and E. Vivo, which made that time in Japan a fantastic one. We didn't meet a Japanese temple, but now Edoardo and I have known how 
is a Japanese party...

About my friends from Vi\c{c}osa, I express my special thanks to Isnard Ferraz and Frederico Vasconcellos. You have transformed the lab. and the moments out of it much nicer. I also thanks all those who have, sincerely, helped me along the way. It includes Pablo Lisboa, Fellipe Rufino, Reinaldo Bastos, Armand Vidal, Alberto Romani and Ismael Carrasco.

Finally, I'm thankful to Prof. S. G. Alves for introducing me in this field two years ago and to
Prof. R. Cuerno for his availability to accept evaluate this dissertation. Unfortunately, the short time that I had for writing it, and boring borucratic problems, prevented out our plans this time.

\vspace{0.5cm}
Thanks the \textit{Coordena\c{c}\~{a}o de Aperfei\c{c}oamento de Pessoal de N\'{\i}vel Superior} (CAPES) by one and half year of Master Scholarship.

==> titulo/titulo_copia.tex <==
\begin{minipage}{110mm}
\centering{
\vspace*{15mm}
\LARGE\textsf{PhD THESIS}
\vspace*{90mm}

\LARGE\textsf{\textbf{Models of social behaviour based}}} \\
\vspace*{5mm}
{\LARGE\textsf{\textbf{on game theory}}}\vspace*{5mm}
\vspace*{40mm}

{\Large\textsf{Jelena Gruji\'c}}
\end{minipage}
\clearemptydoublepage

\thispagestyle{empty}
\vspace*{-15mm}
\begin{minipage}{110mm}
\begin{center}
%\includegraphics[width=30mm]{logouc3m.png}\\[2mm]

{\large \textsf{\textbf{UNIVERSIDAD CARLOS III DE MADRID}}}
\vspace*{18mm}

{\Large\textsf{PhD THESIS}}\vspace*{5mm}
\vspace*{12mm}

{\LARGE\textsf{\textbf{Models of social behaviour based }}} \\
\vspace*{5mm}
{\LARGE\textsf{\textbf{on game theory}}}\vspace*{5mm}

%{The influence of the spatial structure }}}\vspace*{5mm}
%{\LARGE\textsf{\textbf{on cooperation in the}}}\vspace*{5mm}
%{\LARGE\textsf{\textbf{Prisoner's dilemma experiments}}}
\vspace*{10mm}

{\large \textsf{\textit{Author}}}
\vspace*{7mm}

{\Large \textsf{Jelena Gruji\'c}}
\vspace*{10mm}

{\large \textsf{\textit{Supervisors}}}
\vspace*{7mm}

{\Large \textsf{Jos\'e Antonio Cuesta Ruiz \\}} \vspace*{5mm}
{\Large \textsf{ Angel S\'anchez S\'anchez}}
\vspace*{25mm}

%\flushright
%{\large \textsf{Grupo Interdisciplinar de Sistemas Complejos (GISC)\\
%Departamento de Matem\'aticas\\
%Escuela Polit\'ecnica Superior\\
%Universidad Carlos III de Madrid\\[8mm]
%Octubre, 2010}}

{\large \textsf{\textbf{DEPARTMENT OF MATHEMATICS}\\[8mm]
Legan\'es, 2012}}
\end{center}
\end{minipage}


